ReLSO: A Transformer-based Model for Latent Space Optimization and Generation of Proteins

The development of powerful natural language models have increased the ability to learn meaningful representations of protein sequences. In addition, advances in high-throughput mutagenesis, directed evolution, and next-generation sequencing have allowed for the accumulation of large amounts of labeled fitness data. Leveraging these two trends, we introduce Regularized Latent Space Optimization (ReLSO), a deep transformer-based autoencoder which features a highly structured latent space that is trained to jointly generate sequences as well as predict fitness. Through regularized prediction heads, ReLSO introduces a powerful protein sequence encoder and novel approach for efficient fitness landscape traversal. Using ReLSO, we explicitly model the sequence-function landscape of large labeled datasets and generate new molecules by optimizing within the latent space using gradient-based methods. We evaluate this approach on several publicly-available protein datasets, including variant sets of anti-ranibizumab and GFP. We observe a greater sequence optimization efficiency (increase in fitness per optimization step) by ReLSO compared to other approaches, where ReLSO more robustly generates high-fitness sequences. Furthermore, the attention-based relationships learned by the jointly-trained ReLSO models provides a potential avenue towards sequence-level fitness attribution information.

==> sections/related_works.tex <==
\subsection{Related Work}
\label{sec: related-work}

% DL and PROTEIN DESIGN SO FAR
Several deep learning approaches have been proposed in recent years to address the challenge of sequence-based protein design. These methods can be broadly categorized into two groups:

\textbf{Model-based design}: This technique involves training a model to guide the search to better sequences. Two such approaches exist: (1) using the model for \textit{in-silico} screening of candidates, and (2) using the model to directly optimize sequences. The former predominately involves the application of a supervised model $\hat{\phi}$ to predict fitness from sequence, $x$, by learning an approximate mapping $\hat{y} = \hat{\phi}(x)$. After training, this model is used for the \textit{in silico} evaluation of candidate sequences, as part of a search and screen refinement process \cite{Yang:2019ix,biswas2021low}. The latter consists of models that operate directly on sequences with the goal of maximizing a target property \cite{Linder:2020jk}. Model-based design methods have shown promising results in several applications \cite{Linder:2020jk, linder2020fast, liu2020antibody, Valeri:2020kt, angenent2020deep}. Recent efforts haven sought to standardize this approach by introducing a benchmark environment \cite{sinai2020adalead}.

%  <Add sentence or two here about pre-training and its pros/cons>
\textbf{Latent-space optimization}: Another class of deep learning methods for protein design uses generative models to iteratively sample new candidates and select for high-fitness sequences. These methods include DBas \cite{brookes2018design}, which utilizes a batch-wise sampling approach to alternate between sampling and selection steps, resulting in a pool of proposed high-fitness sequences. This method was further enhanced by weighting candidates according to the uncertainty of the generative model and the predictive model used for fitness estimation \cite{brookes2019conditioning}. Most similar to ReLSO in this context is the approach proposed in \cite{tripp2020sample}, where the authors remark that the latent space of a model is often used post-hoc for optimization and may benefit for intentional training or regularization for the task of latent space optimization. In their work this is achieved by retraining a generative model using weighted samples, i.e. placing higher weights on samples that possess the desired trait.

We are also inspired by \cite{gomez2018automatic}, where the model learns a smooth latent space for the optimization of small molecules by jointly training to perform an auxiliary task. We build on their work and that of \cite{castro2020uncovering}, which used the joint training setup to create thermodynamic landscapes of RNA folding, resulting in a smooth latent space amenable to optimization using novel regularizations.  

In contrast to \cite{tripp2020sample} and \cite{brookes2019conditioning}, ReLSO only requires training once and learns a latent space where samples are gradated by fitness. By only requiring a single round of training, ReLSO is better able to leverage gains produced by large, transformer-based models. Furthermore, we depart from the work of \cite{gomez2018automatic} as we extend their training approach to the  protein sequence optimization domain and use a transformer-based encoder. Furthermore, we make use of the gradients provided by the fitness prediction network and highlight it's efficiency in reaching high-fitness sequences.


%\subsection{Protein Design}
%\label{sec: proteindesign}

% PROTEIN DESIGN OVERALL
%Deep learning has found many applications in the field of protein design, in particular sequence-based protein design. In this domain, the prevailing challenge is to design a protein via it's sequence that is optimized for a function such as binding affinity or stability. While physics-based methods currently dominate, a data-driven approach can leverage the greater abundance of labeled data, arising from recent improvements in library generation and phenotypic screening technologies, to learn fundamental, task-specific principles for successful protein design. 

% FITNESS 
%It is important to note that in this work we use the term fitness, $y$, in general to refer to some quantitative level of functionality that a sequence possesses. This can take the form of some biochemical property such as fluorescence, binding affinity, or catalysis. We note that while functionality of a protein sequence is more directly a consequence of the folded, three-dimensional structure of the protein rather than strictly its amino acid sequence, it is often preferable to connect fitness directly to sequence since structural information may not always be available. Indeed, when generating a library of variants, either through a designed, combinatorial approach or by random mutagenesis, it is cost-prohibitive to solve for the structure of each of the $10^{3}$ to $10^{9}$ variants produced. Therefore it is advantageous to extract information about $y$ directly from sequence.

% WHAT PROTEIN DESIGN ACTUALLY IS
%Importantly, protein design is fundamentally a search problem in a complex and vast search space. For most biologically relevant proteins, sequence length can range from few tens to several thousands of residues. Since each position of a $N$-length sequence may contain one of 20 possible amino acids, the resulting combinatorial space (~$20^N$ sequences) is often too large to search exhaustively. Notably this problem arises with the consideration of just canonical amino acids, notwithstanding the growing number of noncanonical alternatives \cite{chen2020engineering}.  A major consequence of the scale of this search space is that most publicly-available datasets, though high-throughout in their scale, capture only a small fraction of possible sequence space and thus the vast majority of possible variants are left unexplored. Within this larger, unexplored space it may be possible to find sequences with higher fitness or more desirable properties for the application of interest. Thus the ability to efficiently search sequence space for high-fitness sequences remains a core problem in protein design.

% EPISTASIS
%Furthermore, a protein sequence determines its function with two notable nuances. First, amino acid residues have can possess important interactions with both sequentially adjacent residues and distant residues, such as with residues comprising structural motifs or functional domains. These long-range dependencies can be challenging to model at the sequence level, as they necessitate some notion of "coupling" between positions far apart. Second, couplings themselves are likely insufficient: past work has shown that protein function is governed by higher-order interactions between residues \cite{russ_evolution-based_2020} (i.e., epistasis) such that the collective effects of mutations can be non-additive and as a result, difficult to predict \cite{pokusaeva_experimental_2019}.

% TRADITIONAL APPROACHES: DIRECTED EVOLUTION, STRUCTURE-BASED
%To navigate protein sequence space, researchers have often utilized an iterative search procedure called directed evolution \cite{arnold_design_1998}. Here libraries of randomized sequences are generated and screened for a function or property of interest. The best sequence or sequences are then carried over to the next round of library generation and selection. Effectively, this searches sequence space using a hill climbing approach and as a consequence, is susceptible to local maxima. Additional approaches to protein design have included structure-based design \cite{rohl_protein_2004,norn_protein_2021} wherein ideal structures are chosen \textit{a priori} and the task is to fit a sequence to the design. With the emergence of powerful deep learning architectures, several promising approaches  to protein design have incorporated models into the design \cite{brookes2018design, brookes2019conditioning}, search \cite{Yang:2019ix, biswas2021low}, or optimization procedure \cite{linder2020fast}.
